Parallel I/O Characterization and Optimization on Large-Scale HPC Systems: A 360-Degree Survey

Driven by artificial intelligence, data science, and high-resolution simulations, I/O workloads and hardware on high-performance computing (HPC) systems have become increasingly complex. This complexity can lead to large I/O overheads and overall performance degradation. These inefficiencies are often mitigated using tools and techniques for characterizing, analyzing, and optimizing the I/O behavior of HPC applications. That said, the myriad number of tools and techniques available makes it challenging to navigate to the best approach. In response, this paper surveys 131 papers from the ACM Digital Library, IEEE Xplore, and other reputable journals to provide a comprehensive analysis, synthesized in the form of a taxonomy, of the current landscape of parallel I/O characterization, analysis, and optimization of large-scale HPC systems. We anticipate that this taxonomy will serve as a valuable resource for enhancing I/O performance of HPC applications.

==> sections/access_patterns.tex <==
% I/O requests by an HPC application can be issued in diverse ways depending on how the application is modeled and coded. Although there is no set definition to describe the access patterns of an application, a lot of research has been done on HPC I/O applications to understand what can constitute an access pattern which includes the number of issued requests, the requests’ sizes, and their spatial location in the file \cite{iosurvey}. These patterns have a direct impact on the overall performance of the application; therefore, it is really important to optimize these data accesses \cite{ioacceleration, patterns}. 

% % There are three classifications of the access patterns: local, global, and system-wide. The local access patterns of an application are in the context of an individual process or a task. They are employed to identify and optimize the client side of the application. The global access pattern looks at all the processes and tasks and is more applicable in optimizing the forwarding layer or the file system as they have a complete picture of all the accesses made by each process. System-wide access patterns look at the access patterns revolving around shared storage infrastructure and the I/O nodes and help optimize the system-wide performance. 

% \subsection{Access Patterns Features}

% In this section, we briefly look at some of the features that can be used to describe an I/O access pattern and their usage in the I/O stack. 

% \paragraph{Operation}

% The first access pattern is the basic I/O operations such as read and write. It also includes the append operation, which performs a write operation to append the data to a file but first positions the file offset at the end of the file using a seek operation. The write operation and the moving of file offset are considered a single atomic operation. 

% \paragraph{File Approach}

% The second access pattern is the way processes perform parallel I/O and how they access the files to read or write data. There can be multiple scenarios in which MPI ranks access the files. The first scenario is the file-per-process approach in which each individual MPI rank writes to an individual file. If the number of processes is too large, a subfiling approach \cite{subfiling} is also used in which data is aggregated into a small subset of processes that access a small number of files. In the second scenario, there is a shared file for all the processes. Typically, in this scenario, there is a single write (commonly rank 0), which receives the data from all the other processes or ranks, aggregates it, and writes it to the shared file. There can also be multiple ranks that aggregate the data and write it to a file. Another approach is to have all the ranks write to pre-defined and non-overlapping locations in a file using implicit coordination.

% % \begin{figure}
% % 	\centering
% % 	\begin{subfigure}{0.80\linewidth}
% % 		\includegraphics[width=\linewidth]{images/file-per-process.png}
% % 		\caption{file-per-process}
% % 		\label{fig:subfigA}
% % 	\end{subfigure}
  	
% %         \begin{subfigure}{0.80\linewidth}
% % 		\includegraphics[width=0.98\columnwidth]{images/Shared file - rank 0.png}
% % 		\caption{Shared file - Rank 0}
% % 		\label{fig:subfigB}
% % 	\end{subfigure}

% %   	\begin{subfigure}{0.80\linewidth}
% % 		\includegraphics[width=0.98\columnwidth]{images/Shared file - aggregators.png}
% % 		\caption{Shared file - Multiple Rank}
% % 		\label{fig:subfigC}
% % 	\end{subfigure}

% %  	\begin{subfigure}{0.80\linewidth}
% % 		\includegraphics[width=0.98\columnwidth]{images/Shared file - coordinated.png}
% % 		\caption{Shared file - Coordinated}
% % 		\label{fig:subfigD}
% % 	\end{subfigure}

% % 	\caption{File approaches for parallel I/O \cite{iosurvey}} 
% % 	\label{fig:file-approaches}
% %          \vspace{-15px}
% % \end{figure}

% \paragraph{Spatial Locality}

% The spatial locality or spatiality has a direct impact on the I/O performance of the application. Spatiality refers to the file offsets between consecutive I/O accesses. There are generally three types of spatial accesses: sequential (contiguous), strided, and random. In sequential or contiguous access, each process accesses the file in contiguous chunks, and that property holds for all the I/O requests. In strided access, chunks of the file are accessed by the process with a fixed-size gap, which is called a stride. After each request, the file pointer is increased by the same size. In random file accesses, the file is accessed randomly without any set pattern. Because of the performance overhead added by random accesses to files, such accesses are not very common in traditional HPC workloads \cite{5222721}. The type of spatial access has a direct correlation with the I/O performance of the application, as the storage hardware and software are directly affected by the data accessed in it. For example, a file system can perform better if the data is accessed in a specific pattern \cite{checkpoint}. 

% % \begin{figure}
% % 	\centering
% % 	\begin{subfigure}{0.98\linewidth}
% % 		\includegraphics[width=0.98\columnwidth]{images/sequential.png}
% % 		\caption{Sequential accesses to a shared file}
% % 		\label{fig:sequential}
% % 	\end{subfigure}
  	
% %         \begin{subfigure}{0.98\linewidth}
% % 		\includegraphics[width=0.98\columnwidth]{images/strided.png}
% % 		\caption{Strided accesses to a shared file}
% % 		\label{fig:strided}
% % 	\end{subfigure}

% %   	\begin{subfigure}{0.98\linewidth}
% % 		\includegraphics[width=0.98\columnwidth]{images/random.png}
% % 		\caption{Random accesses to a shared file}
% % 		\label{fig:random}
% % 	\end{subfigure}

% % 	\caption{Different types of spatial locality \cite{iosurvey}} 
% % 	\label{fig:spatial-locality}
% %          \vspace{-15px}
% % \end{figure}

% \paragraph{Interfaces}

% Interfaces have an important role to play in parallel I/O as they define the APIs and semantics for accessing the data in files. Some of the most common I/O interfaces are POSIX I/O, MPI-IO, and STDIO. POSIX (Portable Operating System Interface) \cite{POSIX} composes a set of standards defined by IEEE to maintain compatibility between different operating systems, which allows an application to run the basic features of an operating system. POSIX also provides an I/O API, called POSIX I/O, to deal with the parallel file system. POSIX I/O introduced asynchronous and synchronous behaviors for local file systems. One of the major advantages of POSIX I/O is that it is highly portable. MPI-IO \cite{MPI-IO} is an extension to the MPI standard and provides an I/O API that comprises the message-passing capabilities of MPI. MPI-IO provides a high-level interface to define the data partitioning among the processes and supports asynchronous I/O. This allows I/O operations to run in parallel with computation. MPI-IO also has relaxed consistency requirements as compared to POSIX. MPI-IO is built on top of ADIO \cite{ADIO}, which is an abstract device interface for parallel I/O. STDIO (Standard I/O library) abstracts all file operations to provide an interface to perform operations on a stream of bytes. It consists of the C \texttt{stdio.h} family of functions such as \texttt{fprintf}, \texttt{fscanf}, \texttt{fopen}, and others \cite{ISO_2020}.

% % Introduced in 1988, However, this portability comes with a price as there are consistency requirements for POSIX write operations in which the application execution has to be stopped for a write call until there is a read call that actually reads the data just written. This introduces complexity in using POSIX I/O for large-scale distributed and parallel file systems as these systems have to adhere to strict consistency requirements using some sort of locking mechanism. This can limit the parallelism of the file system at a large scale. POSIX also leaves the burden of coordinating parallel accesses, buffering, and flushing to the end user which can be problematic for the user if, for example, they are working in a shared-file parallel I/O approach.

% % ADIO implements parallel I/O interfaces portable and efficient by allowing any parallel API to be implemented on top of ADIO. It is not intended to be used directly by programmers and is only an abstraction for building parallel I/O interfaces on top of it. ROMIO \cite{romio} is one such example which is a portable implementation of MPI-IO and uses ADIO to develop this implementation. MPI-IO also provides features related to data access such as blocking or non-blocking and independent or collective accesses. The I/O access patterns generated by MPI-IO are complex and these patterns can be modified as they traverse the stack because of optimizations and transformations made by MPI-IO. 

% % STDIO (Standard I/O library) abstracts all file operations to provide an interface to perform operations on a stream of bytes. It consists of the C stdio.h family of functions such as fprintf, fscanf, fopen etc \cite{ISO_2020}. STDIO does not support random access to data and the application must open a stream, seek to the desired offset, and then read/write the data to the file. STDIO has been increasingly used for various HPC workloads such as in genomics and biology to store sequencing information in textual format \cite{5222721, 10.1145/2749246.2749269}. Even though studies \cite{10.1145/3502181.3531461} have shown that the use of STDIO has increased in supercomputers, it still performs poorly on different transfer sizes on Cori and Summit and hence shows poor I/O performance overall.  

% \paragraph{I/O Mode}

% I/O mode defines how a parallel process accesses a file. There are two I/O modes: individual and collective. In individual mode, each process (MPI rank) accesses the file individually, whereas in collective I/O mode, all the ranks that are accessing the same file issue a single collective call to access that file. Collective I/O is considered a critical optimization in parallel I/O and is readily available in MPI-IO. It is particularly effective when the file accesses of different processes are non-contiguous and interleaved. This mode further allows for optimizations such as collective buffering and data sieving \cite{750599}.

% % Collective I/O mode works in a two-phased strategy. In the first phase which is the communication phase, all the processes participating in the collective I/O call send their data to the "aggregator" nodes. In the I/O phase, the "aggregator" issues the read or write request to the system. This allows larger and contiguous access to the file system even though the individual requests are non-contiguous. One example of a collective I/O function is \texttt{MPI\_File\_write\_at\_all}. Here \texttt{\_all} indicates that all the processes in the MPI communicator will call the write function and \texttt{\_at} indicates that the position in the file is specified as part of the call. 

% % \begin{figure}[h]
% %     \centering
% %     \includegraphics[width=\linewidth]{images/collective.png}
% %     \caption{Basic diagram depicting how collective I/O works}
% %     \label{fig:collective-io}
% % \end{figure}


% \paragraph{Synchronicity}

% Synchronicity deals with how an I/O operation affects the flow of the application. Synchronous or blocking I/O routines halt the execution of the application until the I/O operation is completed. Whereas asynchronous or non-blocking I/O overlaps I/O operations with computation or communication steps, allowing the application execution to progress. Asynchronous I/O provides significant performance speedup when we are accessing large amounts of data. Both POSIX and MPI-IO have support and synchronous and asynchronous I/O. 

% \paragraph{Temporal Behavior}

% Temporal behavior corresponds to the automatic detection of HPC jobs that are not performing well using performance features collected from time-based metrics. There are multiple research works that use such metrics to identify poorly performing HPC jobs as well as detect future performance. Teresa \cite{teresa} is one such tool that uses temporal signatures derived from time-series performance data such as memory and CPU utilization, as well as the number of reads or writes over the disk and network to check if the application's performance is as expected. Omnisc’IO \cite{Omnisc’IO} is another tool that uses a grammar-based I/O model to predict when and where the next I/O operation will occur and how much data will be accessed. It builds the grammar-based I/O model by keeping track of access sizes and offsets and uses that model to make predictions for future requests. 

% \paragraph{Consistency}

% Some research \cite{ISC-paper, 9150354} has been done to check the consistency of the I/O operations to extract meaningful patterns. These works look at the I/O patterns of the application by looking at how many processes read/write to the same file and the order in which these operations occur in a given offset. These patterns also help determine how feasible caching techniques will be. 

\begin{figure*}[!htb]
\resizebox{\linewidth}{!}{

\begin{tikzpicture}[
Models/.style={text centered, text width=2.2cm, font=\bfseries},
attribute/.style={%
grow=down, xshift=0cm,
text centered, text width=2cm,
edge from parent path={(\tikzparentnode.225) |- (\tikzchildnode.west)}},
first/.style    ={level distance=8ex},
second/.style   ={level distance=16ex},
third/.style    ={level distance=24ex},
fourth/.style   ={level distance=32ex},
fifth/.style    ={level distance=40ex},
level 1/.style={sibling distance=10em}]
level 2/.style={sibling distance=5em}]
level 3/.style={sibling distance=5em}]
    % Main Goal
\node[anchor=south]{Access Patterns Features in HPC I/O}
[edge from parent fork down]

% Criteria and Attributes
child{node (model1) [Models] {Operation}
    child[attribute,first]  {node {Read}
                            }
    child[attribute,second] {node {Write}
                                 child[attribute,first]{node {Append}}
                            }
}
%
child{node [Models] {File Approach}
    child[attribute,first]  {node {File-per-process}
     }
    child[attribute,second]  {node {Shared File}
            child[attribute,second]  {node {Rank 0}
                     }
            child[attribute,third]  {node {Multiple Ranks}
                    }
            child[attribute,fourth]  {node {Co-ordinated}
                    }
     }
}
%
child{node [Models] {Spatial Locality}
    child[attribute,first]  {node {Sequential}
          }
    child[attribute,second] {node {Strided}
        }
    child[attribute,third] {node {Random}
        }
}    
%
child{node [Models] {Interfaces}
    child[attribute,first]  {node {POSIX}}
    child[attribute,second]  {node {MPIIO}}
    child[attribute,third]  {node {STDIO}}
 }
child{node [Models] {I/O Mode}
    child[attribute,first]  {node {Individual}
        }
    child[attribute,second]  {node {Collective}
        }
 }
child{node [Models] {Synchronicity}
    child[attribute,first]  {node {Synchronous}}
    child[attribute,second]  {node {Asynchronous}}
 }
child{node [Models] {Temporal Behavior}
    child[attribute,first]  {node {Temporal
                                    Signatures}
        %child[attribute,first]  {node {Teresa \cite{teresa}}
        %}
    }
    child[attribute,second]  {node {Grammar}
       %child[attribute,first]  {node {Omnisc IO \cite{Omnisc’IO}}
       %}                    
    }
}
child{node [Models] {Consistency}
    %child[attribute,first]  {node {I/O Patterns}}
    %}
}
;
\end{tikzpicture}}
\caption{Taxonomy tree defining the access patterns of HPC I/O applications with categories and sub-categories.
\Description{Taxonomy tree defining the access patterns of HPC I/O applications with categories and sub-categories}
\label{fig:access_pattern_tree`}}
\end{figure*}
